Revisiting a Number-Theoretic Puzzle: The Census-Taker Problem

The current work revisits the results of L.F. Meyers and R. See in [3], and presents the census-taker problem as a motivation to introduce the beautiful theory of numbers.

==> graphtex.tex <==
\input graphtex.sty
\endinput
